Generalized Object Detection on Fisheye Cameras for Autonomous Driving: Dataset, Representations and Baseline

Object detection is a comprehensively studied problem in autonomous driving. However, it has been relatively less explored in the case of fisheye cameras. The standard bounding box fails in fisheye cameras due to the strong radial distortion, particularly in the image's periphery. We explore better representations like oriented bounding box, ellipse, and generic polygon for object detection in fisheye images in this work. We use the IoU metric to compare these representations using accurate instance segmentation ground truth. We design a novel curved bounding box model that has optimal properties for fisheye distortion models. We also design a curvature adaptive perimeter sampling method for obtaining polygon vertices, improving relative mAP score by 4.9% compared to uniform sampling. Overall, the proposed polygon model improves mIoU relative accuracy by 40.3%. It is the first detailed study on object detection on fisheye cameras for autonomous driving scenarios to the best of our knowledge. The dataset comprising of 10,000 images along with all the object representations ground truth will be made public to encourage further research. We summarize our work in a short video with qualitative results at https://youtu.be/iLkOzvJpL-A.

==> bib/backup.tex <==
@misc{SLAM,
  title        = {Trained Trajectory based Automated Parking System using Visual SLAM},
  author       = {Nivedita Tripathi and Senthil Yogamani},
  year         = 2020,
  eprint       = {2001.02161},
  archiveprefix = {arXiv},
  primaryclass = {cs.CV}
}
@article{RTT,
  title        = {Randomized kinodynamic planning},
  author       = {LaValle, Steven M and Kuffner Jr, James J},
  year         = 2001,
  journal      = {The international journal of robotics research},
  publisher    = {SAGE Publications},
  volume       = 20,
  number       = 5,
  pages        = {378--400}
}
@inproceedings{deepSemantic_ad,
  title        = {Deep semantic segmentation for automated driving: Taxonomy, roadmap and challenges},
  author       = {Siam, Mennatullah and Elkerdawy, Sara and Jagersand, Martin and Yogamani, Senthil},
  year         = 2017,
  booktitle    = {2017 IEEE 20th international conference on intelligent transportation systems (ITSC)},
  pages        = {1--8},
  organization = {Ieee}
}
@article{modnet,
  title        = {Modnet: Moving object detection network with motion and appearance for autonomous driving},
  author       = {Siam, Mennatullah and Mahgoub, Heba and Zahran, Mohamed and Yogamani, Senthil and Jagersand, Martin and El-Sallab, Ahmad},
  year         = 2017,
  journal      = {arXiv preprint arXiv:1709.04821}
}
@article{soiling,
  title        = {SoilingNet: Soiling Detection on Automotive Surround-View Cameras},
  author       = {Uricar, Michal and Krizek, Pavel and Sistu, Ganesh and Yogamani, Senthil},
  year         = 2019,
  month        = oct,
  journal      = {2019 IEEE Intelligent Transportation Systems Conference (ITSC)},
  publisher    = {Ieee},
  doi          = {10.1109/itsc.2019.8917178},
  isbn         = 9781538670248,
  url          = {http://dx.doi.org/10.1109/ITSC.2019.8917178}
}
@inproceedings{neurall,
  title        = {NeurAll: Towards a Unified Visual Perception Model for Automated Driving},
  author       = {Sistu, Ganesh and Leang, Isabelle and Chennupati, Sumanth and Yogamani, Senthil and Hughes, Ciar{\'a}n and Milz, Stefan and Rawashdeh, Samir},
  year         = 2019,
  booktitle    = {2019 IEEE Intelligent Transportation Systems Conference (ITSC)},
  pages        = {796--803},
  organization = {Ieee}
}
@inproceedings{deep_slam,
  title        = {Visual slam for automated driving: Exploring the applications of deep learning},
  author       = {Milz, Stefan and Arbeiter, Georg and Witt, Christian and Abdallah, Bassam and Yogamani, Senthil},
  year         = 2018,
  booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition Workshops},
  pages        = {247--257}
}
@book{planning,
  title        = {Planning algorithms},
  author       = {LaValle, Steven M},
  year         = 2006,
  publisher    = {Cambridge university press}
}
@article{decision_making,
  title        = {Planning and decision-making for autonomous vehicles},
  author       = {Schwarting, Wilko and Alonso-Mora, Javier and Rus, Daniela},
  year         = 2018,
  journal      = {Annual Review of Control, Robotics, and Autonomous Systems},
  publisher    = {Annual Reviews}
}
@article{woodscape,
  title        = {WoodScape: A Multi-Task, Multi-Camera Fisheye Dataset for Autonomous Driving},
  author       = {Yogamani, Senthil and Hughes, Ciaran and Horgan, Jonathan and Sistu, Ganesh and Chennupati, Sumanth and Uricar, Michal and Milz, Stefan and Simon, Martin and Amende, Karl and Witt, Christian and et al.},
  year         = 2019,
  month        = oct,
  journal      = {2019 IEEE/CVF International Conference on Computer Vision (ICCV)},
  publisher    = {Ieee},
  doi          = {10.1109/iccv.2019.00940},
  isbn         = 9781728148038,
  url          = {http://dx.doi.org/10.1109/ICCV.2019.00940}
}
@article{RCNN,
  title        = {Rich Feature Hierarchies for Accurate Object Detection and Semantic Segmentation},
  author       = {Girshick, Ross and Donahue, Jeff and Darrell, Trevor and Malik, Jitendra},
  year         = 2014,
  month        = jun,
  journal      = {2014 IEEE Conference on Computer Vision and Pattern Recognition},
  publisher    = {Ieee},
  doi          = {10.1109/cvpr.2014.81},
  isbn         = 9781479951185,
  url          = {http://dx.doi.org/10.1109/CVPR.2014.81}
}
@article{kannala2006fisheye,
  author    = {J. Kannala and S.S. Brandt},
  title     = {A generic camera model and calibration method for conventional, wide-angle, and fish-eye lenses},
  journal   = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year      = {2006},
  volume    = {28},
  number    = {8},
  pages     = {1335--1340}
}
@article{LourencoSIFT,
  author    = {Miguel Louren\c{c}o and Joao P. Barreto and Francisco Vasconcelos},
  title     = {{sRD-SIFT:} Keypoint Detection and Matching in Images With Radial Distortion},
  journal   = {IEEE Transactions on Robotics},
  year      = {2012},
  volume    = {28},
  number    = {3},
  pages     = {752--760}
}
@article{hughesFisheye,
  title        = {Equidistant fish-eye perspective with application in distortion centre estimation},
  author       = {Ciaran Hughes and Robert McFeely and Patrick Denny and Martin Glavin and Edward Jones},
  year         = 2010,
  journal      = {Image and Vision Computing},
  volume       = 28,
  pages        = {538--551}
}
@inproceedings{brauerDivisionModel,
  title        = {A new algorithm to correct fish-eye- and strong wide-angle-lens-distortion from single images},
  author       = {Christian Br\"{a}uer-Burchardt and Klaus Voss},
  year         = 2001,
  booktitle    = {IEEE International Conference on Image Processing},
  pages        = {225--228}
}
@inproceedings{scaramuzzaFisheye,
  title        = {A flexible technique for accurate omnidirectional camera calibration and structure from motion},
  author       = {D. Scaramuzza and A. Martinelli and R. Siegwart},
  year         = 2006,
  booktitle    = {IEEE International Conference on Computer Vision Systems}
}
@inproceedings{FasterRCNN,
  title        = {Faster r-cnn: Towards real-time object detection with region proposal networks},
  author       = {Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  year         = 2015,
  booktitle    = {Advances in neural information processing systems},
  pages        = {91--99}
}
@article{he2015spatial,
  title        = {Spatial pyramid pooling in deep convolutional networks for visual recognition},
  author       = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  year         = 2015,
  journal      = {IEEE transactions on pattern analysis and machine intelligence},
  publisher    = {Ieee},
  volume       = 37,
  number       = 9,
  pages        = {1904--1916}
}
@article{FastRCNN,
  title        = {Fast R-CNN},
  author       = {Girshick, Ross},
  year         = 2015,
  month        = dec,
  journal      = {2015 IEEE International Conference on Computer Vision (ICCV)},
  publisher    = {Ieee},
  doi          = {10.1109/iccv.2015.169},
  isbn         = 9781467383912,
  url          = {http://dx.doi.org/10.1109/ICCV.2015.169}
}
@misc{RFCN,
  title        = {R-FCN: Object Detection via Region-based Fully Convolutional Networks},
  author       = {Jifeng Dai and Yi Li and Kaiming He and Jian Sun},
  year         = 2016,
  eprint       = {1605.06409},
  archiveprefix = {arXiv},
  primaryclass = {cs.CV}
}
@article{overfeat,
  title        = {Overfeat: Integrated recognition, localization and detection using convolutional networks},
  author       = {Sermanet, Pierre and Eigen, David and Zhang, Xiang and Mathieu, Micha{\"e}l and Fergus, Rob and LeCun, Yann},
  year         = 2013,
  journal      = {arXiv preprint arXiv:1312.6229}
}
@article{YOLOV1,
  title        = {You Only Look Once: Unified, Real-Time Object Detection},
  author       = {Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
  year         = 2016,
  month        = jun,
  journal      = {2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  publisher    = {Ieee},
  doi          = {10.1109/cvpr.2016.91},
  isbn         = 9781467388511,
  url          = {http://dx.doi.org/10.1109/CVPR.2016.91}
}
@article{YOLO9000,
  title        = {YOLO9000: Better, Faster, Stronger},
  author       = {Redmon, Joseph and Farhadi, Ali},
  year         = 2017,
  month        = jul,
  journal      = {2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  publisher    = {Ieee},
  doi          = {10.1109/cvpr.2017.690},
  isbn         = 9781538604571,
  url          = {http://dx.doi.org/10.1109/CVPR.2017.690}
}
@article{YOLOV3,
  title        = {Yolov3: An incremental improvement},
  author       = {Redmon, Joseph and Farhadi, Ali},
  year         = 2018,
  journal      = {arXiv preprint arXiv:1804.02767}
}
@inproceedings{fasterVSssd,
  title        = {Real-Time Diseases Detection of Grape and Grape Leaves using Faster R-CNN and SSD MobileNet Architectures},
  author       = {Ghoury, Shekofa and Sungur, Cemil and Durdu, Akif},
  year         = 2019,
  month        = {04},
  pages        = {}
}
@inproceedings{ssd,
  title        = {Ssd: Single shot multibox detector},
  author       = {Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C},
  year         = 2016,
  booktitle    = {European conference on computer vision},
  pages        = {21--37},
  organization = {Springer}
}
@article{dssd,
  title        = {Dssd: Deconvolutional single shot detector},
  author       = {Fu, Cheng-Yang and Liu, Wei and Ranga, Ananth and Tyagi, Ambrish and Berg, Alexander C},
  year         = 2017,
  journal      = {arXiv preprint arXiv:1701.06659}
}
@article{mdssd,
  title        = {Mdssd: Multi-scale deconvolutional single shot detector for small objects},
  author       = {Cui, Lisha and Ma, Rui and Lv, Pei and Jiang, Xiaoheng and Gao, Zhimin and Zhou, Bing and Xu, Mingliang},
  year         = 2018,
  journal      = {arXiv preprint arXiv:1805.07009}
}
@article{RetinaNet,
  title        = {Focal Loss for Dense Object Detection},
  author       = {Lin, Tsung-Yi and Goyal, Priya and Girshick, Ross and He, Kaiming and Dollar, Piotr},
  year         = 2017,
  month        = oct,
  journal      = {2017 IEEE International Conference on Computer Vision (ICCV)},
  publisher    = {Ieee},
  doi          = {10.1109/iccv.2017.324},
  isbn         = 9781538610329,
  url          = {http://dx.doi.org/10.1109/ICCV.2017.324}
}
@article{barreto2006unified,
  title        = {Unifying image plane liftings for central catadioptric and dioptric cameras},
  author       = {Barreto, Joao P},
  year         = 2006,
  journal      = {Imaging Beyond the Pinhole Camera},
  publisher    = {Springer},
  pages        = {21–-38}
}
@inproceedings{caruso2015large,
  title        = {Large-scale direct {SLAM} for omnidirectional cameras},
  author       = {Caruso, David and Engel, Jakob and Cremers, Daniel},
  year         = 2015,
  booktitle    = {Proceedinsg of the IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages        = {141--148},
  organization = {Ieee}
}
@article{Khomutenko2016eucm,
  title        = {An Enhanced Unified Camera Model},
  author       = {Bogdan Khomutenko and Gaetan Garcia and Philippe Martinet},
  year         = 2016,
  journal      = {IEEE Robotics and Automation Letters},
  volume       = 1,
  number       = 1,
  pages        = {137--144}
}
@article{MaskRCNN,
  title        = {Mask R-CNN},
  author       = {He, Kaiming and Gkioxari, Georgia and Dollar, Piotr and Girshick, Ross},
  year         = 2017,
  month        = oct,
  journal      = {2017 IEEE International Conference on Computer Vision (ICCV)},
  publisher    = {Ieee},
  doi          = {10.1109/iccv.2017.322},
  isbn         = 9781538610329,
  url          = {http://dx.doi.org/10.1109/ICCV.2017.322}
}
@article{MNC,
  title        = {Instance-Aware Semantic Segmentation via Multi-task Network Cascades},
  author       = {Dai, Jifeng and He, Kaiming and Sun, Jian},
  year         = 2016,
  month        = jun,
  journal      = {2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  publisher    = {Ieee},
  doi          = {10.1109/cvpr.2016.343},
  isbn         = 9781467388511,
  url          = {http://dx.doi.org/10.1109/CVPR.2016.343}
}
@inproceedings{he2016deep,
  title        = {Deep residual learning for image recognition},
  author       = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  year         = 2016,
  booktitle    = {Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages        = {770--778}
}
@inproceedings{polarmask,
  title        = {Polarmask: Single shot instance segmentation with polar representation},
  author       = {Xie, Enze and Sun, Peize and Song, Xiaoge and Wang, Wenhai and Liu, Xuebo and Liang, Ding and Shen, Chunhua and Luo, Ping},
  year         = 2020,
  booktitle    = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages        = {12193--12202}
}
@inproceedings{yoloact,
  title        = {Yolact: Real-time instance segmentation},
  author       = {Bolya, Daniel and Zhou, Chong and Xiao, Fanyi and Lee, Yong Jae},
  year         = 2019,
  booktitle    = {Proceedings of the IEEE international conference on computer vision},
  pages        = {9157--9166}
}
@misc{polyyolo,
  title        = {Poly-YOLO: higher speed, more precise detection and instance segmentation for YOLOv3},
  author       = {Petr Hurtik and Vojtech Molek and Jan Hula and Marek Vajgl and Pavel Vlasanek and Tomas Nejezchleba},
  year         = 2020,
  eprint       = {2005.13243},
  archiveprefix = {arXiv},
  primaryclass = {cs.CV}
}
@article{proposal_free,
  title        = {Proposal-Free Network for Instance-Level Object Segmentation},
  author       = {Liang, Xiaodan and Lin, Liang and Wei, Yunchao and Shen, Xiaohui and Yang, Jianchao and Yan, Shuicheng},
  year         = 2018,
  month        = dec,
  journal      = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  publisher    = {Institute of Electrical and Electronics Engineers (IEEE)},
  volume       = 40,
  number       = 12,
  pages        = {2978–2991},
  doi          = {10.1109/tpami.2017.2775623},
  issn         = {1939-3539},
  url          = {http://dx.doi.org/10.1109/TPAMI.2017.2775623}
}
@article{joint_instance,
  title        = {Instance Segmentation by Jointly Optimizing Spatial Embeddings and Clustering Bandwidth},
  author       = {Neven, Davy and Brabandere, Bert De and Proesmans, Marc and Van Gool, Luc},
  year         = 2019,
  month        = jun,
  journal      = {2019 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  publisher    = {Ieee},
  doi          = {10.1109/cvpr.2019.00904},
  isbn         = 9781728132938,
  url          = {http://dx.doi.org/10.1109/CVPR.2019.00904}
}
@article{pan_deplab,
  title        = {Panoptic-DeepLab: A Simple, Strong, and Fast Baseline for Bottom-Up Panoptic Segmentation},
  author       = {Cheng, Bowen and Collins, Maxwell D. and Zhu, Yukun and Liu, Ting and Huang, Thomas S. and Adam, Hartwig and Chen, Liang-Chieh},
  year         = 2020,
  month        = jun,
  journal      = {2020 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  publisher    = {Ieee},
  doi          = {10.1109/cvpr42600.2020.01249},
  isbn         = 9781728171685,
  url          = {http://dx.doi.org/10.1109/cvpr42600.2020.01249}
}
@inproceedings{OPTICS,
  title        = {OPTICS: Ordering Points to Identify the Clustering Structure},
  author       = {Ankerst, Mihael and Breunig, Markus M. and Kriegel, Hans-Peter and Sander, J\"{o}rg},
  year         = 1999,
  booktitle    = {Proceedings of the 1999 ACM SIGMOD International Conference on Management of Data},
  location     = {Philadelphia, Pennsylvania, USA},
  publisher    = {Association for Computing Machinery},
  address      = {New York, NY, USA},
  series       = {Sigmod '99},
  pages        = {49–60},
  doi          = {10.1145/304182.304187},
  isbn         = 1581130848,
  url          = {https://doi.org/10.1145/304182.304187},
  numpages     = 12,
  keywords     = {database mining, cluster analysis, visualization}
}
@inproceedings{density_cluster,
  title        = {A density-based algorithm for discovering clusters in large spatial databases with noise.},
  author       = {Ester, Martin and Kriegel, Hans-Peter and Sander, J{\"o}rg and Xu, Xiaowei and others},
  year         = 1996,
  booktitle    = {Kdd},
  volume       = 96,
  number       = 34,
  pages        = {226--231}
}
@inproceedings{pytorch,
  title        = {Pytorch: An imperative style, high-performance deep learning library},
  author       = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and others},
  year         = 2019,
  booktitle    = {Advances in neural information processing systems},
  pages        = {8026--8037}
}
@misc{ranger,
  title        = {Gradient Centralization: A New Optimization Technique for Deep Neural Networks},
  author       = {Hongwei Yong and Jianqiang Huang and Xiansheng Hua and Lei Zhang},
  year         = 2020,
  eprint       = {2004.01461},
  archiveprefix = {arXiv},
  primaryclass = {cs.CV}
}
@article{one_cycle,
  title        = {A disciplined approach to neural network hyper-parameters: Part 1--learning rate, batch size, momentum, and weight decay},
  author       = {Smith, Leslie N},
  year         = 2018,
  journal      = {arXiv preprint arXiv:1803.09820}
}
@article{r_adam,
  title        = {On the variance of the adaptive learning rate and beyond},
  author       = {Liu, Liyuan and Jiang, Haoming and He, Pengcheng and Chen, Weizhu and Liu, Xiaodong and Gao, Jianfeng and Han, Jiawei},
  year         = 2019,
  journal      = {arXiv preprint arXiv:1908.03265}
}
@misc{lookahead,
  title        = {Lookahead Optimizer: k steps forward, 1 step back},
  author       = {Michael R. Zhang and James Lucas and Geoffrey Hinton and Jimmy Ba},
  year         = 2019,
  eprint       = {1907.08610},
  archiveprefix = {arXiv},
  primaryclass = {cs.LG}
}
@article{yuvmultinet,
  title        = {YUVMultiNet: Real-time YUV multi-task CNN for autonomous driving},
  author       = {Boulay, Thomas and El-Hachimi, Said and Surisetti, Mani Kumar and Maddu, Pullarao and Kandan, Saranya},
  year         = 2019,
  journal      = {arXiv preprint arXiv:1904.05673}
}
@misc{v3h,
  title        = {R-{Car} {V3H} {System}-on-{Chip} ({SoC})},
  journal      = {Renesas Electronics},
  url          = {https://www.renesas.com/br/en/solutions/automotive/soc/r-car-v3h.html},
  urldate      = {2020-08-24},
  abstract     = {R-Car V3H SoC, part of the Renesas Autonomy platform for ADAS and automated driving, offers high performance computer vision at low power consumption.}
}
@article{agarwal2018recent,
  title        = {Recent advances in object detection in the age of deep convolutional neural networks},
  author       = {Agarwal, Shivang and Terrail, Jean Ogier Du and Jurie, Fr{\'e}d{\'e}ric},
  year         = 2018,
  journal      = {arXiv preprint arXiv:1809.03193}
}
@inproceedings{coors2018spherenet,
  title        = {Spherenet: Learning spherical representations for detection and classification in omnidirectional images},
  author       = {Coors, Benjamin and Paul Condurache, Alexandru and Geiger, Andreas},
  year         = 2018,
  booktitle    = {Proceedings of the European Conference on Computer Vision (ECCV)},
  pages        = {518--533}
}
@article{li2020fisheyedet,
  title        = {FisheyeDet: A Self-Study and Contour-Based Object Detector in Fisheye Images},
  author       = {Li, Tangwei and Tong, Guanjun and Tang, Hongying and Li, Baoqing and Chen, Bo},
  year         = 2020,
  journal      = {IEEE Access},
  publisher    = {Ieee},
  volume       = 8,
  pages        = {71739--71751}
}
@article{teh1989detection,
  title        = {On the detection of dominant points on digital curves},
  author       = {Teh, C-H and Chin, Roland T.},
  year         = 1989,
  journal      = {IEEE Transactions on pattern analysis and machine intelligence},
  publisher    = {Ieee},
  volume       = 11,
  number       = 8,
  pages        = {859--872}
}
@article{perraudin2019deepsphere,
  title        = {DeepSphere: Efficient spherical convolutional neural network with HEALPix sampling for cosmological applications},
  author       = {Perraudin, Nathana{\"e}l and Defferrard, Micha{\"e}l and Kacprzak, Tomasz and Sgier, Raphael},
  year         = 2019,
  journal      = {Astronomy and Computing},
  publisher    = {Elsevier},
  volume       = 27,
  pages        = {130--146}
}
@article{heimberger2017computer,
  title={Computer vision in automated parking systems: Design, implementation and challenges},
  author={Heimberger, Markus and Horgan, Jonathan and Hughes, Ciar{\'a}n and McDonald, John and Yogamani, Senthil},
  journal={Image and Vision Computing},
  volume={68},
  pages={88--101},
  year={2017},
  publisher={Elsevier}
}
@inproceedings{siam2017deep,
  title={Deep semantic segmentation for automated driving: Taxonomy, roadmap and challenges},
  author={Siam, Mennatullah and Elkerdawy, Sara and Jagersand, Martin and Yogamani, Senthil},
  booktitle={2017 IEEE 20th international conference on intelligent transportation systems (ITSC)},
  pages={1--8},
  year={2017},
  organization={IEEE}
}
@inproceedings{kumar2018monocular,
  title={Monocular fisheye camera depth estimation using sparse lidar supervision},
  author={Kumar, Varun Ravi and Milz, Stefan and Witt, Christian and Simon, Martin and Amende, Karl and Petzold, Johannes and Yogamani, Senthil and Pech, Timo},
  booktitle={2018 21st International Conference on Intelligent Transportation Systems (ITSC)},
  pages={2853--2858},
  year={2018},
  organization={IEEE}
}


@article{yahiaoui2019fisheyemodnet,
  title={Fisheyemodnet: Moving object detection on surround-view cameras for autonomous driving},
  author={Yahiaoui, Marie and Rashed, Hazem and Mariotti, Letizia and Sistu, Ganesh and Clancy, Ian and Yahiaoui, Lucie and Kumar, Varun Ravi and Yogamani, Senthil},
  journal={arXiv preprint arXiv:1908.11789},
  year={2019}
}
@inproceedings{horgan2015vision,
  title={Vision-based driver assistance systems: Survey, taxonomy and advances},
  author={Horgan, Jonathan and Hughes, Ciar{\'a}n and McDonald, John and Yogamani, Senthil},
  booktitle={2015 IEEE 18th International Conference on Intelligent Transportation Systems},
  pages={2032--2039},
  year={2015},
  organization={IEEE}
}
@inproceedings{uvrivcavr2019soilingnet,
  title={Soilingnet: Soiling detection on automotive surround-view cameras},
  author={U{\v{r}}i{\v{c}}{\'a}{\v{r}}, Michal and K{\v{r}}{\'\i}{\v{z}}ek, Pavel and Sistu, Ganesh and Yogamani, Senthil},
  booktitle={2019 IEEE Intelligent Transportation Systems Conference (ITSC)},
  pages={67--72},
  year={2019},
  organization={IEEE}
}


@inproceedings{kumar2020fisheyedistancenet,
  title={Fisheyedistancenet: Self-supervised scale-aware distance estimation using monocular fisheye camera for autonomous driving},
  author={Kumar, Varun Ravi and Hiremath, Sandesh Athni and Bach, Markus and Milz, Stefan and Witt, Christian and Pinard, Cl{\'e}ment and Yogamani, Senthil and M{\"a}der, Patrick},
  booktitle={2020 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={574--581},
  year={2020},
  organization={IEEE}
}
@article{kumar2020unrectdepthnet,
  title={UnRectDepthNet: Self-Supervised Monocular Depth Estimation using a Generic Framework for Handling Common Camera Distortion Models},
  author={Kumar, Varun Ravi and Yogamani, Senthil and Bach, Markus and Witt, Christian and Milz, Stefan and Mader, Patrick},
  journal={arXiv preprint arXiv:2007.06676},
  year={2020}
}





@inproceedings{su2019kernel,
  title        = {Kernel transformer networks for compact spherical convolution},
  author       = {Su, Yu-Chuan and Grauman, Kristen},
  year         = 2019,
  booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages        = {9442--9451}
}
@article{jiang2019spherical,
  title        = {Spherical CNNs on unstructured grids},
  author       = {Jiang, Chiyu and Huang, Jingwei and Kashinath, Karthik and Marcus, Philip and Niessner, Matthias and others},
  year         = 2019,
  journal      = {arXiv preprint arXiv:1901.02039}
}
@article{everingham2010pascal,
  title        = {The pascal visual object classes (voc) challenge},
  author       = {Everingham, Mark and Van Gool, Luc and Williams, Christopher KI and Winn, John and Zisserman, Andrew},
  year         = 2010,
  journal      = {International journal of computer vision},
  publisher    = {Springer},
  volume       = 88,
  number       = 2,
  pages        = {303--338}
}
@article{khomutenko2015enhanced,
  title        = {An enhanced unified camera model},
  author       = {Khomutenko, Bogdan and Garcia, Gaetan and Martinet, Philippe},
  year         = 2015,
  journal      = {IEEE Robotics and Automation Letters},
  publisher    = {Ieee},
  volume       = 1,
  number       = 1,
  pages        = {137--144}
}
@article{dong2020ellipse,
  title        = {Ellipse R-CNN: Learning to Infer Elliptical Object from Clustering and Occlusion},
  author       = {Dong, Wenbo and Roy, Pravakar and Peng, Cheng and Isler, Volkan},
  year         = 2020,
  journal      = {arXiv preprint arXiv:2001.11584}
}
@book{kaehler2016learning,
  title        = {Learning OpenCV 3: computer vision in C++ with the OpenCV library},
  author       = {Kaehler, Adrian and Bradski, Gary},
  year         = 2016,
  publisher    = {" O'Reilly Media, Inc."}
}
@inproceedings{Geiger2012CVPR,
  title        = {Are we ready for Autonomous Driving? The KITTI Vision Benchmark Suite},
  author       = {Andreas Geiger and Philip Lenz and Raquel Urtasun},
  year         = 2012,
  booktitle    = {Conference on Computer Vision and Pattern Recognition (CVPR)}
}
@inproceedings{lienhart2002extended,
  title        = {An extended set of haar-like features for rapid object detection},
  author       = {Lienhart, Rainer and Maydt, Jochen},
  year         = 2002,
  booktitle    = {Proceedings. international conference on image processing},
  volume       = 1,
  pages        = {I--i},
  organization = {Ieee}
}
@article{douglas1973algorithms,
  title        = {Algorithms for the reduction of the number of points required to represent a digitized line or its caricature},
  author       = {Douglas, David H and Peucker, Thomas K},
  year         = 1973,
  journal      = {Cartographica: the international journal for geographic information and geovisualization},
  publisher    = {University of Toronto Press},
  volume       = 10,
  number       = 2,
  pages        = {112--122}
}


==> include/commented.tex <==
%INTRODUCTION
When an autonomous vehicle travels from source to destination, a navigator such as google maps or HD Maps generates a high-level route. A series of connected nodes at finite distances make up this route. The vehicle moves from one node to another in a repetitive way until it reaches the destination. The sensing stage collects information about the surroundings via sensors such as Camera, LiDAR, RADAR, and Ultrasonic sensors. 
Perception involves the extraction of useful information from the raw data like lane positions, pedestrians, and other vehicles~\cite{deepSemantic_ad}, moving objects detection~\cite{modnet} and recognition of drivable regions. Localization is the vehicle's ability to precisely know its position in the real world at decimeter accuracy~\cite{SLAM, deep_slam}. In simple words, perception answers what is around the vehicle, and localization answers precisely where the vehicle is. Path planning algorithms~\cite{planning} make use of this related information to define a path to navigate from one node to another.\par
%-------------------------------------------------------------------------
The fact is, there is no ideal projection or correction. These corrections are application-driven, and every correction technique has its disadvantages. Rectilinear correction suffers from loss of Field of View (FoV) and sampling issues, Piece-wise linear with artifacts at transition areas and massive bleeding in the image, and Cylindrical as a quasi-linear correction offers a practical trade-off.  Another overhead is extra computational resources needed for correction, as the visual perception pipeline usually has different algorithms demanding different view projections.
Though Look Up Tables (LUTs) make this correction process accelerated, LUTs rely on an online calibration that needs to be generated every time there is a change in the online calibration. Despite these disadvantages, image correction is encouraged due to the non or early deep learning object recognition and segmentation algorithms' limitations. With a push in deep neural networks, this trend is slowly changing.
Modern CNN based object detection algorithms like YOLO and FasterRCNN can detect objects on raw fisheye images. The main issue with object detection on raw fisheye images is the representation of objects as bounding boxes.\par
Objects go through severe deformations due to radial distortion in fisheye images, and box representation fails in many practical scenarios. \varun{Where are those 2 cars coming into the paper from?} For instance, if two parked cars have a free slot in between, they are detected and localized by a conventional bounding box. The boxes of the side cars will be incorrectly intersecting with the free slot. This will cause inaccurate footpoint computation and might cause incorrect decisions to be taken by the autonomous vehicle. These scenarios motivate the need for accurate representation in fisheye-based visual navigation systems. A full-fledged solution to this problem is instance segmentation. However, most state-of-the-art algorithms, such as MaskRCNN, demand higher computing powers. They are unrealistic to work on low-power hardware used in  Level 2 and 3 autonomous vehicles. Henceforth, there is a need for memory and computation efficient models, motivating us to build our architecture on YOLO characteristics, and study various real-time fisheye object detection representations.
%-------------------------------------------------------------------------
\textbf{\textit{Surround View cameras}}
Typically, automotive systems use a multi-camera network. Current systems have at least four cameras, and it is increasing to more than ten cameras for future generation systems. Figure~\ref{fig:car_new} illustrates the camera mounting locations on the car, where it spans over the entire 360$^{\circ}$ field-of-view surrounding the car. The four cameras' geometric structure and the car's motion induces a Spatio-temporal structure across the four images.
For example, when the car is turning left, the front camera's region imaged by the right-mirror camera after a delay. There is also a similarity in the near-field road surface in all the four cameras as they belong to the same road surface.
Surround-view cameras are focused on near field sensing and typically used for low-speed applications like parking and traffic jam assist~\cite{heimberger2017computer}.\par
%-------------------------------------------------------------------------
\begin{figure}[t]
\captionsetup{singlelinecheck=false, font=small,  belowskip=-12pt}
centering
\includegraphics[width=0.45\textwidth]{img/undist.jpg}
\caption{\textbf{Undistorting the fisheye image:} (a) Rectilinear correction; (b) Piecewise linear correction; (c) Cylindrical correction. \textbf{Left:} Raw image and \textbf{Right:} Undistorted image.}
\label{fig:projections}
\end{figure}
%-------------------------------------------------------------------------
\textbf{\textit{Object Detection}} is the first and foremost problem in visual perception. which involves recognizing and localizing the objects in the image. Hence object detection models' performance directly influence the success and failure of autonomous driving systems. A simple and common representation of objects in images is bounding box representation.
State-of-the-art methods for object detection based on deep learning can be broadly classified into two types, two-stage detectors, and single-stage detectors.
%-------------------------------------------------------------------------
\begin{figure*}
\captionsetup{singlelinecheck=false, font=small,  belowskip=-12pt}
\centering
\includegraphics[width=0.99\linewidth]{img/representation_failure_case.jpg}.
\caption{\varun{FIND A BETTER IMAGE. RIGHT ONE IS COMPRESSED!}\textbf{Parking spot failure case}. \textbf{Left:} Bounding box incorrectly intrudes with a free parking spot. \textbf{Right:} Accurate instance mask provides accurate representation allowing the parking spot to be reported as free.}
\label{fig:parking_failure}
\end{figure*}
% ------------------------------------------------------------------------
\textbf{\textit{Two Stage Object Detection}}
In two-stage approaches, object detection is split into two tasks,
(i) Extraction of Region of Interest (ROI)s
(ii) Regression for bounding boxes in these ROIs using CNN features.
RCNN~\cite{RCNN} was the first approach to employ this technique. In the first stage, selective search is used to propose ROIs, followed by a CNN feature extraction. In the second stage, an SVM is trained to classify the objects based on the CNN features. Further improvements have been deployed on two-stage networks. For instance, Region Proposal Network (RPN) were introduced in~\cite{FasterRCNN}, which made end-to-end training possible with high accuracy. 
% ------------------------------------------------------------------------
\textbf{\textit{Single Stage Object Detection}}
In single-stage approaches, RoI extraction is eliminated where classification and regression of bounding boxes are done directly on CNN feature maps. YOLO~\cite{YOLOV1} is a well-known algorithm that divides the input image into grids and predicts bounding boxes directly by regression and classification at each grid.
In~\cite{YOLO9000}, the performance was further improved by introducing batch normalization and replacing fully connected layers with anchor boxes for bounding box prediction. Anchor boxes are computed over the dataset, representing the average variation of height and width of the dataset's objects. Instead of directly regressing for object width and height, YOLOv2 predicts off-sets from a predetermined set of anchors with particular height-width ratios.
Further improvement has been proposed in ~\cite{YOLO9000} and ~\cite{YOLOV3}. Darknet-53 has been used as a feature extraction backbone and multi-scale prediction approach providing real-time performance in~\cite{YOLOV3}.\par
%-------------------------------------------------------------------------
\textbf{\textit{Instance Segmentation}} comprises predicting both object bounding box and pixel-level object mask. Instance segmentation can be modeled as a bounding box detection followed by a binary segmentation within the box. This approach has been adopted by \cite{MaskRCNN} where an additional decoder for object mask segmentation was added to \cite{FasterRCNN}. Segmentation is performed as a binary classification to differentiate object pixels from the background or other object pixels. 
Multi-task Network Cascade (MNC)~\cite{MNC} uses a similar approach to MaskRCNN. It uses RPN for box proposals, followed by class agnostic instances on the proposed regions and, finally, categorical classification of these mask instances.
On the other hand, single-shot instance segmentation has been explored by~\cite{yoloact} uses a single encoder dual parallel decoder style architecture for instance-level image segmentation. Two parallel branches are proposed generating prototypes and linear coefficients in a parallel mechanism. Both are combined later to provide the final predictions. Instead of dense pixels prediction for each mask, another approach has recently gained attention, such as PolarMask~\cite{polarmask} and PolyYOLO~\cite{polyyolo}, which predict only the object contour. Such approaches eliminate the computational overhead for useless pixel-wise classification.
%-------------------------------------------------------------------------
\section{Object Detection on Fisheye Cameras}

Fisheye cameras make use of non-linear mapping to generate a large field of view. With just four surround-view fisheye cameras, a dense $360\degree$ near field perception can be achieved, making them suitable for automated parking, low-speed maneuvering, and emergency braking. This advantage comes at the cost of non-linear distortions in the image. Objects at different angles from the image center look quite different, making the object detection a challenge. A common practice is to rectify distortions in the image by a 4\textsuperscript{th} order polynomial model or Unified camera model. The fact is, there is no ideal projection or correction. These corrections are application-driven, and every correction technique has its disadvantages (Figure \ref{fig:projections}). Rectilinear correction suffers from loss of Field of View (FoV) and sampling issues, Piece-wise linear with artifacts at transition areas and massive bleeding in the image, and Cylindrical as a quasi-linear correction offers a practical trade-off.  Another overhead is extra computational resources needed for correction, as the visual perception pipeline usually has different algorithms demanding different view projections. Though Look Up Tables (LUTs) make this correction process accelerated, LUTs rely on an online calibration that needs to be generated every time there is a change in the online calibration. Despite these disadvantages, image correction is encouraged due to the non or early deep learning object recognition and segmentation algorithms' limitations. With a push in deep neural networks, this trend is slowly changing. Modern CNN based object detection algorithms like YOLO and FasterRCNN can detect objects on raw fisheye images. The main issue with object detection on raw fisheye images is the representation of objects as bounding boxes.\par
%-------------------------------------------------------------------------
\textbf{\textit{Bounding boxes on Fisheye}}
Objects go through serious deformations due to radial distortion in fisheye images, and box representation fails in many practical scenarios. For instance, Figure \ref{fig:parking_failure} shows an automated car maneuvering to a parking slot between the two cars. Two cars got detected and localized by a conventional bounding box. However, only in instance segmentation case objects are located correctly outside the free parking spot. Using standard box, objects seem to be present inside the parking spot, and hence the free parking spot is incorrectly reported as unavailable spot. These cases motivate the need for correct representation in fisheye-based visual navigation systems. A full-fledged solution to this problem is instance segmentation. However, most state-of-the-art algorithms, such as MaskRCNN, demand higher computing powers. They are unrealistic to work on low-power hardware that is generally used in  2 and Level 3 autonomous vehicles. Hence there is a need for memory and computation efficient models, which motivates us to build our architecture on YOLO style and study various representations for real-time fisheye object detection.\par
% METHOD-------------------------------------------------------------------------
\begin{figure}
   \captionsetup{singlelinecheck=false, font=small,  belowskip=-12pt}
   \centering
   \includegraphics[width=0.99\linewidth]{img/dense_vs_sapse.pdf}
   \includegraphics[width=0.48\textwidth]{img/fixed_vs_variable_step_2.jpg}
   \caption{Illustration of three types of sampling of polygon vertices on the object contour - (1) Uniform sampling on object contour, (2) Uniform sampling of polar angle, and (3) Variable step representation to maximize utilization of vertices according to curvature.}
   \label{fig:fixed_vs_variable_step}
\end{figure}
%-------------------------------------------------------------------------
We explore ellipse representation for various reasons. Unlike circles, an ellipse has two radii, which help minimize the area inside it to fit the whole object. Moreover, Ellipse has no corners. It helps in minimizing occlusions with the neighboring objects as well as the area included inside it. 
(3) Ellipse can be represented using the exact five parameters of an oriented bounding box, including ($\hat{x}$, $\hat{y}$, $\hat{w}$, $\hat{h}$, $\hat{\theta}$).
Hence, ellipse representation is efficient and easy to learn using a standard object detection algorithm. We use the same loss function that is used in oriented box representation.

This method is generic for any object contour and it is calibration-agnostic. 
Moreover, the parameters can be used to train a CNN to learn them directly; hence, \textit{we plan to publicly release our generated representations upon acceptance of this paper to motivate CNN construction to learn them directly}.\par
In terms of the curved bounding box, we don't exploit additional restrictions in the perspective of fisheye cameras. The perspective of fisheye cameras is discussed in more detail in \cite{hughesFisheye}, and further investigation here may lead to a reduced parameter space for the curved bounding box fitting. This remains future work.\par
%-------------------------------------------------------------------------
\subsection{Generic Polygon Representations}

We explore the object's polygon-based instance segmentation to maximize the overlap between the prediction and the mask annotation. Unlike conventional instance segmentation techniques, which perform pixel-wise classification, we focused on obtaining the object contour points only to maximize the model speed for real-time performance. We generated annotations of two categories, one, polar representation for the contour points, and the other is a Cartesian representation. \\
Instead of massive backbone architecture, we employed lightweight ResNet-18 as our encoder. These changes enabled us to develop a small footprint instance segmentation model with just ~13M parameters. We enhanced this baseline model to perform object detection for different representations. Our model is quite suitable for real-time applications such as object detection on Level-3 automotive ECUs. Keeping the network architecture similar in all experiments resulted in a fair comparison between these different representations.\par
%-------------------------------------------------------------------------
Using variable-step provides significantly higher accuracy than fixed-step with improvement of 28\% in IoU with instance mask. This approach makes a 4-sided polygon have better accuracy than a 24-point polygon with fixed-step which demonstrates the effectiveness of our method in simplifying the representation while obtaining the best accuracy. 
We apply the same algorithm on 24-point polygon and we achieve 9\% improvement in accuracy over the fixed-step 24-point model which is the best result we obtained. We continue generating our data using variable-step representation based on these results. We predict two Cartesian coordinates ($x$, $y$) per object point, where each point is represented relative to the grid cell during training. Using this model, we provide a comparison between arbitrary 4-points polygon vs. conventional bounding box in Table~\ref{tab:gt_table} as both have the same number of points.  We observe similar performance between fixed-step Cartesian representation and polar representation, with higher accuracy using variable-step representation as reported in Table~\ref{tab:gt_table}. 
In Table~\ref{tab:prediction_table}, we report the results using the best model for polygon representation, which is a variable-step polygon using 24 points.\par
%-------------------------------------------------------------------------
% EXPERIMENTS
\begin{figure}[t]
   \captionsetup{singlelinecheck=false, font=small,  belowskip=-12pt}
   \centering
   \includegraphics[width=0.48\textwidth]{img/rv_vs_side_analysis_2.jpg}
   \caption{\textbf{Top:} FV and RV cameras in an AD scene show small distortion in the objects of interest, especially in the center of the image. The standard box in green is almost the same as the oriented box in blue for objects with minimal distortion, resulting in a small angle of the oriented box (around +-10degrees in most cases). \textbf{Bottom:} Higher distortion is observed in side cameras as the objects are distributed in a broader range of the street. Angles in side cameras are steeper than angles in front and rear ones where there is a more considerable difference observed between the green box and the blue box. Angle values are in the range of +-40 to +-90 degrees due to heavy distortion. 
   \textbf{Bottom:} Data analysis shows that our data is mainly dominated by horizontal objects of angles close to 0, which is the case where there is almost no difference between standard and oriented boxes. \sy{remove graph, it is against our motivation for different representations}
   }
 \label{fig:rv_vs_side_cam_analysis}
 \end{figure}
%-------------------------------------------------------------------------
To evaluate the representations, we first generate ground truth for the different representations, and we evaluate their IoU vs. instance mask to obtain the upper bound performance. Second, we construct CNN networks, train them using the generated annotation, and evaluate our prediction vs. the instance segmentation contour. This is to evaluate the impact of added inaccuracy due to the training process. 
The bounding boxes have steeper angles in the side cameras relative to the front and rear cameras. In front and rear cameras, many objects can be represented by horizontal or vertical boxes, which is the case where there is no difference between an oriented box and a standard box, for instance. For that reason.\par

\subsection{Footpoint Metric}
In previous subsection, we discussed mIOU metric which enables comparison of different representations on the image plane. However, this is not suitable from the application perspective of autonomous driving. Objects detected are mapped to a fusion map which is typically a 2D top view grid map. Figure \ref{fig:footpoint_example} illustrates this with an example. The pedestrians detected are shown with uncertainty in the top view. From this perspective, it is more important to localize the objects in this map coordinate system than accurately bound the object with a representation.
%-------------------------------------------------------------------------
 \begin{figure}[t]
   \captionsetup{singlelinecheck=false, font=small,  belowskip=-12pt}
   \centering
   \includegraphics[width=0.5\textwidth]{img/pd.png}
   \caption{Illustration of world footpoint.}
 \label{fig:footpoint_example}
 \end{figure}
%-------------------------------------------------------------------------
\begin{figure}[t]
   \captionsetup{singlelinecheck=false, font=small,  belowskip=-12pt}
   \centering
   \includegraphics[width=0.5\textwidth]{img/footpoint.png}
   \caption{Distribution of objects in the world.}
 \label{fig:footpoint_distribution}
 \end{figure}
%-------------------------------------------------------------------------
